Magnetization reversal in FePt thin films: Experiments and simulations

The competition between shape and perpendicular magnetic anisotropies (PMA) in magnetic thin films gives rise to unusual magnetic behaviors. In ferromagnetic films with moderate PMA the magnetic domain configuration transitions from planar to stripe-like domains above a critical thickness, $t_c$. In this article, we present a detailed study of the magnetization switching mechanism in FePt thin films, where this phenomenon is observed. Using micromagnetic simulations and experiments, we found that below $t_c$ the reversal mechanism is well described by the two-phase model while above this thickness the magnetization within each stripe reverses by coherent rotation. We also analyzed the PMA and its temperature dependence, probing that substrate-induced strains are responsible for the abnormal coercive field behavior observed for FePt films with $t>t_c$.

==> captions.tex <==
\section*{Figures}
\begin{figure}[ht]
\centering
%\includegraphics[width=\textwidth]{Figure1.eps}

\caption{\label{FePt_TEM}(a) Cross sectional HR-TEM image and (b) SAED pattern from a 40 nm thickness FePt film deposited on a silicon substrate. White circles indicate ordered regions of the sample}
\end{figure}

\begin{figure}[ht]
\centering
%\subfloat{\includegraphics[width=0.5\textwidth]{Figure2a.eps}}
%\subfloat{\includegraphics[width=0.5\textwidth]{Figure2b.eps}}
\caption {\label{XRD_PSI_RT}(a) XRD patterns of FePt(60nm)/Si recorded for $\theta/ 2\theta$ for $\psi =0$ and $\psi = 70$. (b) Calculated average crystallite size using the Scherrer equation and the width of the (111) reflection vs the film thickness for FePt on silicon.}
\end{figure}

\begin{figure}[ht]
\centering
%\subfloat{\hspace*{-0.4cm}\includegraphics[width=0.535\textwidth]{Figure3a.eps}}\hspace*{-0.4cm}
%\subfloat{\hspace*{-0.4cm}\includegraphics[width=0.535\textwidth]{Figure3b.eps}}\\
%\subfloat{\includegraphics[width=0.5\textwidth]{Figure3c.eps}}
%\subfloat{\includegraphics[width=0.5\textwidth]{Figure3d.eps}}
\caption{\label{M_H_MFM}In-plane easy axis $(\varphi=0^0)$. hysteresis loops and MFM images for FePt films of (a, c) $t=10$ nm and (b, d) $t=60$ nm, respectively. All the measurements were performed at $T=300$ K. 
}
\end{figure}

\begin{figure}[ht]
\centering
%\subfloat{\includegraphics[width=0.593\textwidth]{Figure4a.eps}}
%\begin{minipage}[b]{0.407\textwidth}
%\includegraphics[width=\textwidth]{Figure4b.eps}\
%\includegraphics[width=\textwidth]{Figure4c.eps}
%\end{minipage}
\caption{\label{Mr_angular_10nm}(a) Hysteresis loops measured for $\varphi=0^0$ and $\varphi=90^0$ for FePt(10 nm)/Si. (b)  angular dependence of the remanent magnetization. (c) Angular dependence of the coercive field for a 10 nm thickness FePt thin film plotted together with the magnetization reversal models: Stoner-Wohlfarth, Kondorsky and two phase model.
}
\end{figure}

%\begin{figure}[ht]
%\centering
%\includegraphics[width=\textwidth]{Diapositiva8.JPG}
%\caption{\label{Hc_angular_10nm}}
%\end{figure}
%\
\begin{figure}[ht]
%\centering
%\subfloat{\includegraphics[width=0.45\textwidth]{Figure5a.eps}}
%\subfloat{\includegraphics[width=0.54\textwidth]{Figure5b.eps}}
%\includegraphics[width=\textwidth]{MFM_vs_campo.jpg}
\caption{\label{MFM_vs_H} (a) MFM image of a representative FePt film with an external magnetic field applied along the direction parallel to the stripes. (b) Stripe-domains period ($\lambda_S$) calculated from MFM images as a function of the magnetic field.
}
\end{figure}

\begin{figure}[ht]
\centering
%\includegraphics[width=\textwidth]{Figure6.eps}
%\includegraphics[width=\textwidth]{Figure6.JPG}
\caption{\label{Sim60} Experimental and simulated hysteresis loops of a FePt 60 nm/Si.  (1-5) Domain structure as a function of magnetic field. Detail of the evolution of the magnetization within a stripe and y-z crossection as a function of magnetic field.}
\end{figure}

\begin{figure}[ht]
\centering
%\subfloat{\includegraphics[width=0.5\textwidth]{Figure7a.eps}}
%\subfloat{\includegraphics[width=0.5\textwidth]{Figure7c.eps}}\\
%\subfloat{\includegraphics[width=0.5\textwidth]{Figure7b.eps}}
%\subfloat{\includegraphics[width=0.5\textwidth]{Figure7d.eps}}
\caption{\label{perfil_mz_mx} (a) $m_z$ and (b) $m_x$ profile along Y axis for a 60 nm FePt thin film simulated at remanence. Detail of the magnetic field dependence of the (c) $m_z$ and (d) $m_x$ profile.}
\end{figure}

\begin{figure}[ht]
\centering
%\includegraphics[width=\textwidth]{Figure8.eps}
\caption{\label{Hc_T}Temperature dependence of the coercive field for 60 and 10 nm thickness FePt films.
}
\end{figure}

\begin{figure}[ht]
\centering
%\includegraphics[width=\textwidth]{Figure9.eps}
%\includegraphics[width=\textwidth]{Diapositiva16.JPG}
\caption{\label{MFM_T}MFM images measured at (a) T=77 K and (b)T=300 K for a representative FePt film.
}
\end{figure}

\begin{figure}[ht]
\centering
%\includegraphics[width=\textwidth]{Figure10.eps}
\caption{\label{d_111_vs_T} (a) d(111) temperature dependence for different XRD geometries. (b) difference between nearly inplane interplannar distance and out of plane interplannar distance.
}
\end{figure}

\begin{figure}[ht]
%\subfloat{\includegraphics[width=0.8\textwidth]{Figure11ab.eps}\hspace{-1cm}}
%\begin{minipage}[b]{0.25\linewidth}
%\includegraphics[width=\textwidth]{Figure11c.eps}\vspace{-0.1cm}\\
%\includegraphics[width=\textwidth]{Figure11d.eps}
%\vspace{0.2cm}
%\end{minipage}
\caption{\label{Sim_vs_KPMA}Simulated (a) remanence and (b) coercive field as a function of the magnetic anisotropy constant for a 60 nm FePt film. Simulated magnetic domain configuration for (c) $K_{PMA}=0.9$ $\mathrm{\frac{Merg}{cm^3}}$ and (d) $K_{PMA}=1.6$ $\mathrm{\frac{Merg}{cm^3}}$.}
\end{figure}

\begin{figure}[ht]
%\centering
%\includegraphics[width=\textwidth]{Figure12.eps}
\caption{\label{ciclos_sim_KPMA}Simulated hysteresis loops from a 60 nm FePt film with ($\blacksquare$) 0.9 $\mathrm{\frac{Merg}{cm^3}}$ and (\textcolor{red}{$\bullet$}) 1.6 $\mathrm{\frac{Merg}{cm^3}}$ perpendicular magnetic anisotropy constant.
}
\end{figure}

\begin{figure}[ht]
\centering
%\includegraphics[width=\textwidth]{Figure13.eps}
\caption{\label{Inversion_SIM_vs_t}Simulated time evolution of the magnetic domain configuration from a 60 nm FePt film with (a-d) $K_{PMA}=0.9$ $\mathrm{\frac{Merg}{cm^3}}$ and (e-h) $K_{PMA}=1.6$ $\mathrm{\frac{Merg}{cm^3}}$.}
\end{figure}


